Compositionality Through Language Transmission, using Artificial Neural Networks

We propose an architecture and process for using the Iterated Learning Model ("ILM") for artificial neural networks. We show that ILM does not lead to the same clear compositionality as observed using DCGs, but does lead to a modest improvement in compositionality, as measured by holdout accuracy and topologic similarity. We show that ILM can lead to an anti-correlation between holdout accuracy and topologic rho. We demonstrate that ILM can increase compositionality when using non-symbolic high-dimensional images as input.

==> 5c_experiment3.tex <==
\section {Experiment 2: Sampling from Teacher}

In the experiments above, the teacher utterances are sampled deterministically. Given a set of meanings, in this case images, the utterances generated by the teacher are deterministic, conditional on the current learned model. We investigate the effect of using sampling from the teacher logits, as a categorical distribution, rather than taking the argmax. Our hypothesis, following the results of \citet{st2019} for self-training, is that adding additional noise might improve compositionality in ILM.

Table \ref{tab:results_opengl_temperature} shows the effect of teacher sampling temperature, for the 2 shapes dataset. We report results after using ILM for 2 generations. We can see that adding sampling reduces the holdout accuracy, but does improve holdout rho. It is interesting that there is an anti-correlation between topographic similarity and holdout accuracy. We note that topographic similarity depends uniquely on the compositionality of the utterances, i.e. on the compositional behavior of the sender. Holdout accuracy depends also on the compositional behavior of the receiver. Based on tologophical rho, on the holdout set, it looks like sampling utterances from the teacher increases the compositionality of the teacher. However, this comes at the cost of reducing holdout accuracy, which drops quite considerably. One hypothesis could be that adding noise to the teacher reduces the compositional behavior of the student. However, it could also be that the additional noise in the teacher simply confuses the student, 


% Next, we observe that sampling from the teacher, rather than using the argmax language, appears to increase the compositionality of the sender, but reduce the compositionality of the receiver.

% Thus, compositionality, as measured by topological similarity, does increase.

\begin{table}[h]
\small
\centering
    \begin{tabular}{lll}
    \toprule
Temp & Holdout acc & Holdout rho \\
\midrule
0 (argmax) & \textbf{0.52+/-0.04} & 0.33+/-0.02 \\
0.00001 &  &  \\
0.1 & 0.12+/-0.03 & 0.25+/-0.05 \\
0.5 & 0.13+/-0.04 & 0.3+/-0.1 \\
1 & 0.17+/-0.03 & \textbf{0.5+/-0.1} \\
1.5 & 0.12+/-0.02 & 0.4+/-0.2 \\
\bottomrule
\end{tabular}
    \caption{
    Effect of teacher sampling temperature, using OpenGL dataset.
    Results for OpenGL 2 shapes dataset. 'Temp' is sampling temperature.}
    \label{tab:results_opengl_temperature} 
\end{table}

